Dynamic Anchor Selection and Real-Time Pose Prediction for Ultra-wideband Tagless Gate

Ultra-wideband (UWB) is emerging as a promising solution that can realize proximity services, such as UWB tagless gate (UTG), thanks to centimeter-level localization accuracy based on two different ranging methods such as downlink time-difference of arrival (DL-TDoA) and double-sided two-way ranging (DS-TWR). The UTG is a UWB-based proximity service that provides a seamless gate pass system without requiring real-time mobile device (MD) tapping. The location of MD is calculated using DL-TDoA, and the MD communicates with the nearest UTG using DS-TWR to open the gate. Therefore, the knowledge about the exact location of MD is the main challenge of UTG, and hence we provide the solutions for both DL-TDoA and DS-TWR. In this paper, we propose dynamic anchor selection for extremely accurate DL-TDoA localization and pose prediction for DS-TWR, called DynaPose. The pose is defined as the actual location of MD on the human body, which affects the localization accuracy. DynaPose is based on line-of-sight (LOS) and non-LOS (NLOS) classification using deep learning for anchor selection and pose prediction. Deep learning models use the UWB channel impulse response and the inertial measurement unit embedded in the smartphone. DynaPose is implemented on Samsung Galaxy Note20 Ultra and Qorvo UWB board to show the feasibility and applicability. DynaPose achieves a LOS/NLOS classification accuracy of 0.984, 62% higher DL-TDoA localization accuracy, and ultimately detects four different poses with an accuracy of 0.961 in real-time.

==> 6_discussions.tex <==
\section{Discussion and Future Work}
\label{sec:discussion}

\noindent\textbf{One device operation:} The current implementation uses Qorvo UWB board because there is no Android Open Source Project (AOSP) API to obtain CIR information from UWB module.
UWB modules of Samsung flagship smartphones are currently NXP chipset, and hence we have to implement all the architecture of {\pp} if CIR related API is provided.
Therefore, we currently communicate with NXP developers to add the features, such as CIR and channel diagnostics, to NXP chipset and we expect {\pp} can be implemented in Samsung devices without extra 3rd party UWB module in a few months.

\noindent\textbf{Pilot for UTG:}
We already finished the implementation and showed the feasibility with PoC.
Therefore, the next step for UTG is to pilot to get feedback from real customers.
To do this, we collaborate with GeoPlan, which is the company that provides UWB positioning services in Korea.
We provide the application of {\pp} and GeoPlan support the equipment such as UTG and NXP UWB modules, and have plans for experiment together before pilot.
The pilot will be conducted in Seoul Station targeted for the employees of the station.
